Balancing expressiveness and inexpressiveness in view design

We study the design of data publishing mechanisms that allow a collection of autonomous distributed datasources to collaborate to support queries. A common mechanism for data publishing is via views: functions that expose derived data to users, usually specified as declarative queries. Our autonomy assumption is that the views must be on individual sources, but with the intention of supporting integrated queries. In deciding what data to expose to users, two considerations must be balanced. The views must be sufficiently expressive to support queries that users want to ask -- the utility of the publishing mechanism. But there may also be some expressiveness restriction. Here we consider two restrictions, a minimal information requirement, saying that the views should reveal as little as possible while supporting the utility query, and a non-disclosure requirement, formalizing the need to prevent external users from computing information that data owners do not want revealed. We investigate the problem of designing views that satisfy both an expressiveness and an inexpressiveness requirement, for views in a restricted declarative language (conjunctive queries), and for arbitrary views.

==> app-localgen.tex <==
\subsection*{Proof in generality of Theorem \ref{thm:ucqsufficeslocal}}

\michael{Needs to be checked again}

Recall that in the body we claimed that for any local constraints
$\Sigma$, if there are views
that are useful for CQ $\util$ and non-disclosing for
CQ $\secret$, we can find such views that are CCQs.
We now sketch the argument for this.
It might be helpful for the reader to look at the case of
TGDs in the body, and consider how this might be generalized
to disjunctive TGDs. 

Note that global $Q$-$\Sigma$-equivalence, as defined as in the TGD case within
the body, is still the coarsest equivalence relation that is useful. That
is, the analog of 
Proposition \ref{prop:qequivcoarse} from the body still holds in the
presence of arbitrary local constraints.
Thus if any view is useful and non-disclosing then global $Q$-$\Sigma$-equivalence
is an abstract view that is useful and non-disclosing.

Fixing source $s$, along with two instances $\inst_1$ and $\inst_2$
for source $s$ satisfying $\Sigma$. We say that the instances
are $\Sigma$ shuffle-equivalent if:

\emph{Whenever} we have an $s$-context $C$ satisfying $\Sigma$, 
and a binding $\sigma$ of  the $s$ source-join variables
in $C$ such that   $C, \sigma \models \canonctxt^s(Q)$
%,the overlap
of $C$ and $\inst_1$ is included in the image of $\sigma$, 
and
$\inst_1, \sigma \models \canonview^s(Q)$.


\emph{Then}  for some shuffle $\shuf$ such that  $C$ also satisfies
$\shuf(\canonctxt^s(Q))$ we have
$\inst_2, \sigma$ satisfies $\shuf(\canonview(Q))$.

We justify this definition by showing the
analog of Proposition \ref{prop:shuffleequivqequiv}:

\begin{proposition} \label{prop:shuffleequivqequivgen}
$\Sigma$ shuffle-equivalence is the same as global $Q$-equivalence.
\end{proposition}


\begin{proof}
Suppose $s$-instances $\inst_1$ and $\inst_2$ satisfying $\Sigma$ are $\Sigma$-$(s,Q)$-equivalent;
that is, they agree when paired with any context satisfying $\Sigma$.
Fix a variable binding $\sigma$ for $\sjvars(s,Q)$  along
with an $s$-context $C$.
 Then $(\inst_1,C) \models Q$.
By  $\Sigma$-$(s,Q)$-equivalence $(\inst_2,C) \models Q$ via some homomorphism
$h$, which must map the source-join variables to elements in the image
of $\sigma$. Create a shuffle $\shuf$ such that
when  $\shuf(x_i)=x_j$ we have  $\sigma(x_j)=h(x_i)$.
It is easy to verify that this shuffle suffices.

In the other direction, suppose $\inst_1$ and $\inst_2$ are $\Sigma$ shuffle-equivalent,
and consider a context $C$ satisfying $\Sigma$
such that $(\inst_1, C) \models Q$ via some homomorphism
of $h$. 
Let $\sigma$ be the restriction
of $h$ to $\sjvars(s,Q)$. 
Thus there  is $\shuf$ such that $C, \sigma$ satisfies $\shuf(\canonctxt^s(Q))$
and $\inst_2, \sigma \models \shuf(\canonview(Q))$.
Thus $(\inst_2,C) \models Q$.
\end{proof}


For a source $s$ and type $\tau$,
an \emph{$s,\tau$ test} is an $s$-context $\inst'$ 
that satisfies $\Sigma$ along with a homomorphism $h'$
of $\canonctxt^{s}(Q)$ into $\inst'$ whose restriction $\sigma$ to the source-join variables
of $s$ satisfies $\tau$.
An \emph{$s,\tau$ assortment} is any function taking  each $s, \tau$ test  to
a shuffle $\shuf$ such that there is a homomorphism of
$\shuf(\canonctxt^{s}(Q))$ into $\inst'$ extending $\sigma$.
Note that the identity is always one such shuffle.


Fixing still a source $s$ and  type $\tau$, we let the
view $V_{\tau, s}$ be  the disjunction over all possible assortments of
the conjunction of $\shuf(\canonview^s(Q))$ where the conjunction
is over the shuffles $\shuf$ in the image of the assortment.
Note that even though the assortment is infinite, its image is a collection of shuffles,
and hence is finite.

We complete our proof of Theorem 
\ref{thm:ucqsufficeslocal}
by showing  that these views capture $\Sigma$-shuffle equivalence.

\begin{proposition} \label{prop:shuffleequivviewequivgen}
Two instances are $\Sigma$-shuffle equivalent if and only if they agree on
each $V_{\tau, s}$.
\end{proposition}
\begin{proof}
In one direction, suppose $\inst_1$ and $\inst_2$ are $\Sigma$-shuffle equivalent, and
suppose $\sigma$ is an output of $V_{\tau, s}$ on $\inst_1$. We aim to show $\sigma$
is an output of the view on $\inst_2$.
There is an assortment $\assort$ that witnesses that $\sigma$ is an output of the view.
Thus for each test $C, h$  with $\assort(C,h)=\shuf$ we have
$\inst_1, \sigma \models \shuf(\canonview^s(Q)$.
This implies that $\inst_1, \shuf(\sigma) \models \canonview^s(Q)$
while $C, \shuf(\sigma) \models \canonctxt^s(Q)$.
Applying $\Sigma$-shuffle equivalence to 
$C$ we know that there is
$\shuf'$,  depending on the test, such that
$\inst_2, \shuf(\sigma)  \models  \shuf'(\canonview^s(Q))$ and
$C, \shuf(\sigma) \models \shuf'(\canonview^s(Q))$.
Now define an assortment by mapping a given $C, h$ to
$\shuf'(\shuf)$. This witnesses that $\sigma$ is an output of the
view on $\inst_2$.



In the other direction, suppose $\inst_1$ and $\inst_2$ agree on the views.
Fix an $s$-context $C$ satisfying $\Sigma$ 
 and $\sigma$ a binding for the $s$ source-join variables
in $C$ such that   $C, \sigma \models \canonctxt^s(Q)$,
 the overlap
of $C$ and $\inst_1$ is included in the image of $\sigma$, and
$\inst_1, \sigma \models \canonview^s(Q)$.
Let $\tau$ be the type of $\sigma$.
We have a homomorphism $h$ extending $\sigma$ witnessing that $C, \sigma \models \canonctxt^s(Q)$.
Thus $(C, h)$ is an $s, \tau$ test, and we can extend it to an $s, \tau$ assortment $\assort$ arbitrarily
(e.g. using the identity on the other tests).
%view conjoins over the models in an assortment; disjoin over assortments.
%want to claim that $\sigma$ is in the view image; seems ok, since for the identity it is easy.
Since $\inst_2$ and $\inst_1$ agree on the views, there is another assortment $\assort'$ such
that $\sigma$ is in the disjunct of the view corresponding to $\assort'$ on $\inst_2$.
In particular, considering the test $(C,h)$  there is a shuffle $\shuf'$ such
that $C, \sigma \models \shuf'(\canonctxt^s(Q)$ and $\inst_2 \models \shuf'(\canonview^s(Q))$.
But this is as  required for $\Sigma$-shuffle equivalence.
\end{proof}

Putting together the propositions above, as in the setting without
constraints, completes the proof of Theorem \ref{thm:ucqsufficeslocal}.


==> app-replicationeasycase.tex <==
In the case of two sources, we can state a converse to 
Proposition \ref{prop:fullrep}.

If no replicated predicate occurs in $\utility$,
we can characterize the design problem using a simple case analysis. 
If no predicate replicated between the two sources
occurs in $\secret$, then the replication constraint is clearly irrelevant.  We can simply
eliminate the replicated predicates from the schema and consider the corresponding problem
with the constraints dropped.
If some replicated predicate $R$ occurs in $\secret$ but not in $\utility$, then
the canonical d-view of $\utility$ are
UN non-disclosing for $\secret$. For any global instance $\globinst$, we can consider $\globinst'$
that is identical to $\globinst$ except $R$ is empty (in all sources). Then $\globinst'$
clearly agrees with $\globinst$ on the canonical d-view of $\utility$, and
does not satisfy $\secret$.
%thus we only have to worry about the case where a predicate satisfying a replication constraint
%occurs in $\utility$








==> app-specialcases.tex <==

\subsection*{Proof of Proposition \ref{prop:monfrontier1}}
Recall the statement:

\medskip

If $Q$ is a monadic frontier CQ, then 
for any source $s$ and
for any two $s$-instances $\inst_1$ and $\inst_2$,
if $\inst_1$ and $\inst_2$ are   $(s,Q)$-equivalent, then $\inst_1$ and $\inst_2$ agree
on $\canonview^s(Q)$.

\medskip

\begin{proof}
If $\inst_1$ and $\inst_2$ are $(s,Q)$-equivalent then by Proposition
\ref{prop:fullshuffle} they agree on the full shuffle views.
%$\fullshuff(\canonview^s(Q))$.
But in the monadic frontier case the full shuffle is just %$\fullshuff(\canonview^s(Q))= 
$\canonview^s(Q)$.
\end{proof}

\subsection*{Proof of Proposition \ref{prop:monfrontier2}} 
Recall the statement:

\medskip

Suppose $Q$ is a monadic frontier CQ, and we have
arbitrary views $\varb$ that determine $Q$.  Then $\varb$ determines
each $\canonview^s(Q)$. In particular, if $\varb$ is non-disclosing
for some CQ $\secret$, then so are the canonical
views.

\medskip

\begin{proof}
Consider  $\inst_1$ and $\inst_2$ over source $s$ that
agree on $\varb$. By Proposition \ref{prop:qequivcoarse}, $\inst_1$ and $\inst_2$
are globally $Q$-equivalent, and thus by Proposition \ref{prop:monfrontier1} they
agree on $\canonview^s(Q)$.
\end{proof}



==> counterexamplearbviews.tex <==
\begin{example} \label{ex:arbviews}
The following example shows that even when we cannot get useful
and non-disclosing CQ views, we may be able to obtain
useful and non-disclosing views in a richer language.

Consider a d-schema with two sources, one containing ternary relation $R$ and the other containing
unary relation $S$.
Let $\util=\exists x_1 ~  x_2 ~ y ~ R(x_1, x_2, y) \wedge R(y, x_2, x_1) \wedge S(x_1) \wedge S(x_2)$
and $\secret= \exists x ~ R(x,x,x)$.  

Observe that:

\begin{compactenum}
\item $\util$ is minimal: clearly neither of the $R$ atoms can be dropped,
and neither $S$ atom can be dropped either.

\item The canonical d-view of $\util$ is UN disclosing for $\secret$.

The canonical view for the $R$ source
is $\exists y ~ R(x_1,x_2, y) \wedge R(y, x_2, x_1$.
Consider the critical instance. 
%Recall that this is the instance
%consisting of a single element $\critelement$, where every relation
%holds.
An external party  will know
that the instance contains $\{R(\critelement,\critelement,y_0),
R(y_0,\critelement,\critelement)\}$ for some 
$y_0$. On the other hand,
if $y_0$ was unequal to $\critelement$, then the views
would reveal $x_1=y_0, x_2=\critelement$. So $y_0$ must be $\critelement$,
and therefore $\secret$ is disclosed.

\end{compactenum}

Using the above two observations and our prior results, we
know that no CQ views can be UN non-disclosing for $\secret$ and useful
for $\util$. We will now show that there is an arbitrary view
that is UN non-disclosing for $\secret$ and useful for $\util$.


However, we will show later (Example \ref{ex:invshuffleviews})
that if we allow either DCQs or queries with negation,
then we can find views that are useful for $\util$ and UN non-disclosing for $\secret$.
\myeat{
there are 
Consider the views that reveal all of $S$,  i.e.  $V_S(x)=S(x)$, 
and also the following two views on $R$:

\begin{align*}
VR_1(x)= \{ x  \mid ~ \exists y ~ R(x, x, y) \wedge R(y, x, x)\} \\
VR_2(x_1, x_2) = \\
 \{x_1, x_2  \mid ~ \exists y ~R(x_1,x_2, y) \wedge R(y, x_2, x_1) \wedge y \neq x_2 \}
\end{align*}

We argue that these views are useful and UN non-disclosing.
For UN non-disclosure, consider the following transformation $T$ on any
instance $R_0$ of the $R$-source:
$T$ takes any fact of the form $R(c,c,c)$
and replaces it with two
facts $R(d, c, c)$ and $R(c, c, d)$ where $d$ is not
in the domain of $R_0$. Note that in particular $d \neq c$.
One can see that given a d-instance $\globalinst=(R_0, S_0)$, the instance $(T(R_0), S_0)$
for $T$ above
is  indistinguishable from $\globalinst$, and does not satisfy $\secret$; therefore
 the views are UN non-disclosing.

We now show that the views are useful
for $\util$.  Suppose $\globalinst$ and $\globalinst'$ are indistinguishable and $\globalinst$
has a match of $\util$. Let $R(c_1, c_2, d)$ and $R(d, c_2, c_1)$ be the witness to this
match in $\globalinst$.
First suppose $d \neq c_2$. Then due to indistinguishability in $VR_2$ we have the
same facts in $\globalinst'$ and hence also have a match of $\util$.
If $d=c_2$, then due to indistinguishability in $VR_1$ we have the same
facts in $\globalinst'$ and hence also have a match.
}
%note that the last paragraph is the place where we used the presence of both $S(x_1) S(x_2)$
%in the query in the query is important
\end{example}



 


==> finalexample.tex <==
\begin{example} \label{ex:nonlocalconstraints}
We give an example of the power of Theorem \ref{thm:fullrep}.
Consider two sources $R$ and $S$. The $R$-source contains
relations $R_1$ and $R_2$. The $S$-source
contains relations $S_1$ and $S_2$.
The utility and the secret queries, as well as the intersource constraints are:
\begin{align*}
	\util=\exists x,y. R_2(x,y) \wedge R_1(x,y) \wedge S_2(x,y) \\
	\secret= \exists x. R_2(x,x) ~~~~~
	\Sigma= \{\forall x,y. R_1(x,y) \leftrightarrow S_1(x,y) \}
\end{align*}
We can see that the canonical d-view of $\util$ is UN disclosing
for $\secret$.

Below, we show that there exists a set of views that are useful for $Q$ and non-disclosing for $p$. 
First, we define a transformation $\stretchf_R$ from $R$-instances into $R$-instances. 
The transformation replaces each tuple ${(c_j,c_k) \in \inst_R(R_i)}$, for each ${1 \leq i \leq 2}$, 
by ${(c_j, c_{k+1})}$, if ${j \leq k}$ and by ${(c_{j+1}, c_k)}$, if ${j > k}$.
We analogously define a transformation 
$\stretchf_S$ from $S$-instances to $S$-instances. 
For each ${i \geq 0}$, let $\stretchf^i_R$ (resp. $\stretchf^i_S$) be the result of applying $\stretchf_R$ (resp. $\stretchf_S$) $i$ times.
We can see that (i) $\stretchf_R$ produces instances not satisfying $\secret$ and (ii)
for each ${i \geq 0}$ and ${\globinst=(\inst_R, \inst_S)}$,
$\globinst$ has a match of $\util$ iff  
$(\stretchf^i_R(\inst_R), \stretchf^i_S(\inst_S))$ has a match of $\util$.
Furthermore, for any two valid d-instances
${(\inst_R, \inst_S)}$ and ${(\inst'_R, \inst'_S)}$ with
non-empty local instances, we have: (iii)
if ${\inst_R=\stretchf^i_R(\inst'_R)}$, then ${\inst_S=\stretchf^i_S(\inst'_S)}$ and vice versa; 
similarly, if ${\inst'_R=\stretchf^i_R(\inst_R)}$, then ${\inst'_S=\stretchf^i_S(\inst_S)}$ and vice versa. 
Property (iii) holds due to $\Sigma$: if property (iii) did not hold, then 
${\inst_R(R_1) \neq \inst_S(S_1)}$ violating $\Sigma$. 

Let $\equiv_R$ be the coarsest equivalence relation which relates
each $\inst$ and $\inst'$ such that one is $\stretchf$ of the other.
We define $\equiv_S$ analogously. Finally, we define the view
$\equiv_0$ consisting of $\equiv_R$ and $\equiv_S$.

We claim that $\equiv_0$ is UN non-disclosing
for $\secret$ and useful for $\util$.
For UN non-disclosure, consider an arbitrary d-instance $\globalinst=(\inst_R, \inst_S)$ that
satisfies $\Sigma$. Then the instance
$(\stretchf^i_R(\inst_R), \stretchf^i_S(\inst_S))$, for ${i \geq 0}$
is $\equiv_0$ to $\globalinst$ (by definition), does not satisfy $\secret$ (due to property (i)) 
and satisfies $\Sigma$ (due to property (ii)).
Regarding utility, $\equiv_0$ is useful for $\util$ due to properties (ii) and (iii). 
\end{example}


==> introalt.tex <==
\section{Introduction} \label{sec:intro}
The value of data is increased when data owners
make their data  available through publicly-accessible
interfaces. The value is magnified even further
when multiple  data owners publish information from related
datasets; this allows users to answer queries that require
linking information across datasources.

But the benefits  of data publishing come with a corresponding
risk of revealing too much.  For example, here may be information
that a data owner wishes to protect, and a user
may be able to infer this information either
from the published data in isolation, or from the
data published by all parties as a whole.
There is thus a need to provide data publishing mechanisms
that are simultaneously expressive enough to be useful -- they enable users
to answer appropriate queries -- while satisfying some expressiveness restriction.


In data publishing much of the  focus
has been on disclosure via the familiar  mechanism of
\emph{views} -- declarative queries whose
output is made available to users as a table. 
In this context the competing requirements on
a publishing mechanism have been primarily studied in isolation.
There is  extensive work on analysis
of the utility of a set of views: namely given a query, can it be answered
using the views, see, e.g. \cite{DBLP:journals/vldb/Halevy01,DBLP:journals/jcss/CalvaneseGLR12}.
There has also been research concerning analysis
of whether a given set of views 
obeys some expressiveness \emph{restriction}. The negation of answerability
is clearly too weak a restriction, since it just
guarantees that on some instance the query answer can not be computed from the view
images. 
%Similarly, analysis of answerability on a given source \cite{authorizationviews,abiteboulduschka} is not sufficient for privacy.
A relevant query-based notion of expressiveness  restriction is \emph{data-independent privacy}:
given the views and a set of  ``secret'' queries, check that the secret query answers
can not be computed from the views on any source data. Variants of this problem have been studied in
\cite{dnprivacy,lics16,privacyjair,ijcai19}. Expressiveness restrictions with a similar
flavor have also been studied in the context of ontologies \cite{DBLP:conf/semweb/BonattiS13}.
But the question of whether there is a query-independent expressiveness restriction appropriate
for views based on traditional database queries, as well as the question of how one obtains views that satisfy both
expressiveness and inexpressiveness requirements,
has not been considered 
in the context of traditional queries and views, to the best of our knowledge. 



\myeat{
In the multi-agent systems community there is 
%work concerning
%``secure aggregation of distributed information'' \cite{sadi}. This is
work concerned with  protocols allowing a set of agents to learn a distribution
on source data
without revealing certain local information (e.g. \cite{sadi}). The notion of security is ``exact and
information-theoretic'', as in this work:  they deal
with getting the exact answer to a query using a deterministic algorithm, but without restricting the computational power used in answering. 
But the setting, unlike in this work,  is propositional.
}

A larger body of work comes from privacy research, considering the design
of mechanisms  achieving a mix of expressiveness (``utility'') and inexpressiveness
(``privacy'') goals. But the focus
is  on 
probabilistic transformations or, more generally, probabilistic
protocols (see e.g. \cite{infotheoreticprivccd,diffpriv,diffprivj}). The guarantees are probabilistic,
 sometimes alternatively or additionally
with computational restrictions on an external party.
%Instead of just deterministically
%outputing some data, 
\myeat{
Probabilistic protocols iterate rounds of messages,
either broadcast to all owners or point-to-point between data owners. The behavior of the protocol
includes randomization, which allows the mechanisms
to achieve very strong privacy guarantees. In particular
they can achieve guarantees that do not require the specification of a privacy goal in terms of a specific set of 
protected queries. 
For example, in  information-theoretic privacy (e.g. \cite{infotheoreticprivccd})  the goal
is a mechanism that can guarantee  that any data owner ``learns nothing'' (in probabilistic terms) from
a run of the protocol that they cannot learn from the answer to the utility
query in isolation. Research
 in \emph{differential privacy} \cite{diffpriv,diffprivj} has introduced mechanisms
that  guarantee that the probability of an output will not be impacted (up to
some $\epsilon$ that is a parameter to the analysis) by the presence or absence
of any tuple in the database.  Roughly speaking, the attacker will learn nothing
about any ground fact in the database.
}
\myeat{Recent efforts \cite{pricingprivate} have considered a family of mechanisms that 
look at database queries, with the utility of a mechanism defined (as in our case)
using the notion of query determinacy. But randomness still plays a central
role in the mechanism and in the definition of privacy.}


In contrast, we consider the question of designing views that use \emph{traditional database queries},
with no randomization,  so that
 conflicting requirements of expressiveness and inexpressiveness are satisfied. Both our expressiveness
and inexpressiveness requirements will be given in terms of \emph{exact information-theoretic criteria}:
they will be defined in terms of what queries can be answered exactly (as opposed
to probabilistically)  by a party with unlimited computation power. Due both to the difference in the mechanisms
we consider and the requirements we impose,
our contribution has a very different flavor  from  prior lines of work.
\myeat{
It also differs from work on secure querying over distributed data \cite{jenniesecurequery}.
There the goal is to support ad hoc querying of traditional database queries in the presence
of privacy restrictions; but they allow the use of encryption as a query language primitive.
}




\input{runningexample}
Our goal here is to look at the problem of designing 
independent views over multiple relational datasources that satisfy both expressiveness and
inexpressiveness requirements.
Our expressiveness requirement (usefulness) will be phrased in terms of the ability to answer  a 
relational query, where answering is the traditional deterministic notion used in database theory and KR.
For expressiveness limitations we require the views to be
useful but to \emph{minimize information} within a class of views.
We also consider an  expressiveness limitation specified by  \emph{non-disclosure} of 
a  set of \emph{secret queries}. Our contributions include formalizing these notions,
characterizing when minimal information views exist and what form they take, and determining
when views exist that satisfy utility and expressiveness limitations. We look at these problems
both for views given in the standard view language of conjunctive queries, and for arbitrary views.
We also consider the impact of background knowledge on these problems.






==> replication-idea.tex <==
Before giving the argument formally, 
we give the basic idea of how to exploit replication,
which is to take the data and apply a translation
to all the values. In each source, the views will output \emph{all iterated translations
of the data}: see Figure \ref{fig:replication}. An external entity will not know
that the data is one of the infinitely many iterates, but will not be able to determine
which iterate corresponds to the source data. Since the value of the replicated relation (thick lines
in Figure \ref{fig:replication}) is synched between sources,
the set of possible d-instances is not the product of the  interates given by each source, but rather
consists of all iterates of the true d-instance. Using the properties of the translation,
we can show that the value of the utility query $\util$ is the same on all these possible instances.

\begin{figure}[hbt]
\centering
\includegraphics[width=8cm]{replication.pdf}
\caption{Exploiting Replicatons}
\label{fig:replication}
\end{figure}


==> specialcasesarbviews.tex <==
%Cases where Qequiv implies Canonview equivalence -- e.g. monadic frontier.

\subsection{Special cases}
Given a d-schema and a CQ $Q$ over it, we say 
$\util$ is \emph{monadic frontier} if for every source $s$, $\sjvars(s,\util)$
 has at most one free variable in it.
We note that $(s,Q)$ equivalence degenerates to agreement on the canonical views
under this condition.

\begin{proposition} \label{prop:monfrontier1} If $Q$ is a monadic frontier CQ, then 
for any source $s$ and
for any two $s$-instances $\inst_1$ and $\inst_2$,
if $\inst_1$ and $\inst_2$ are   $(s,Q)$-equivalent, then $\inst_1$ and $\inst_2$ agree
on $\canonview^s(Q)$.
\end{proposition}
\myeat{
\begin{proof}
If $\inst_1$ and $\inst_2$ are $(s,Q)$-equivalent then by Proposition
\ref{prop:fullshuffle} they agree on the full shuffle views.
%$\fullshuff(\canonview^s(Q))$.
But in the monadic frontier case the full shuffle is just %$\fullshuff(\canonview^s(Q))= 
$\canonview^s(Q)$.
\end{proof}
}

Using prior results, it follows that under this restriction 
using arbitrary views does not make view design any easier:

\begin{proposition} \label{prop:monfrontier2} Suppose $Q$ is a monadic frontier CQ, and we have
arbitrary views $\varb$ that determine $Q$.  Then $\varb$ determines
each $\canonview^s(Q)$. In particular, if $\varb$ is non-disclosing
for some CQ $\secret$, then so are the canonical
views.
\end{proposition}
\myeat{
\begin{proof}
Consider  $\inst_1$ and $\inst_2$ over source $s$ that
agree on $\varb$. By Proposition \ref{prop:qequivcoarse}, $\inst_1$ and $\inst_2$
are $Q$-equivalent, and thus by Proposition \ref{prop:monfrontier1} they
agree on $\canonview^s(Q)$.
\end{proof}
}

The same argument holds for any CQ for which \emph{there is only one invariant shuffle}.
The special case applies to Example \ref{ex:run}, implying  that \emph{no useful  and
non-disclosing set of views exist} for this case.


